Adaptive Reconvergence-driven AIG Rewriting via Strategy Learning

Rewriting is a common procedure in logic synthesis aimed at improving the performance, power, and area (PPA) of circuits. The traditional reconvergence-driven And-Inverter Graph (AIG) rewriting method focuses solely on optimizing the reconvergence cone through Boolean algebra minimization. However, there exist opportunities to incorporate other node-rewriting algorithms that are better suited for specific cones. In this paper, we propose an adaptive reconvergence-driven AIG rewriting algorithm that combines two key techniques: multi-strategy-based AIG rewriting and strategy learning-based algorithm selection. The multi-strategy-based rewriting method expands upon the traditional approach by incorporating support for multi-node-rewriting algorithms, thus expanding the optimization space. Additionally, the strategy learning-based algorithm selection method determines the most suitable node-rewriting algorithm for a given cone. Experimental results demonstrate that our proposed method yields a significant average improvement of 5.567\% in size and 5.327\% in depth.

==> sections/experiment.tex <==
\section{experiment}
\label{sec:experiment}

\subsection{Setup}
We use the well-known EPFL logic synthesis benchmark suite as benchmarks, which serves as a comparative standard for benchmarking logic optimization algorithms. All experiments have been conducted on an Intel(R) Xeon(R) Gold 6252 CPU @ 2.10GHz. The correctness of the results has been verified using combinational equivalence checking implemented in ABC.

\subsection{Evaluation of single operator optimization quality}
\subsubsection{}
\subsubsection{}

Table II shows the results of optimizing the AIG network. The table lists the results of the ABC rewrite and refactor algorithms, as well as the results of an exact synthesis algorithm developed in date2020. For each case, the table lists the area and depth after one optimization iteration, as well as the improvement rate for each indicator. It can be seen that our average area improvement rate is 5.18\%, surpassing date2020 and coming in second to the rewriting algorithm. The average depth improvement rate is 5.69\%, significantly exceeding the rewrite and refactor algorithms, but date2020 does not list this data.   \\


% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[thp]
\centering
\caption{Comparison the result of operators with preserving depth.}
\label{table:opt_preserve_depth}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|cc|cccc|cccc|cc|cccc|}
	\hline
	\multirow{2}{*}{}         & \multirow{2}{*}{name} & \multicolumn{2}{c|}{origin} & \multicolumn{4}{c|}{rewrite} & \multicolumn{4}{c|}{refactor} & \multicolumn{2}{c|}{date20} & \multicolumn{4}{c|}{ours}                                                                                                                                                                                                                                                                    \\ \cline{3-18}
	                          &                       & \multicolumn{1}{c|}{area}   & depth                        & \multicolumn{1}{c|}{area}     & \multicolumn{1}{c|}{a\%}    & \multicolumn{1}{c|}{depth} & d\%   & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{depth} & d\%  & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{depth} & d\%   \\ \hline
	\multirow{10}{*}{arith}   & log2                  & \multicolumn{1}{c|}{32060}  & 444                          & \multicolumn{1}{c|}{31547}    & \multicolumn{1}{c|}{1.60}   & \multicolumn{1}{c|}{443}   & 0.23  & \multicolumn{1}{c|}{31521}  & \multicolumn{1}{c|}{1.68}  & \multicolumn{1}{c|}{444}   & 0    & \multicolumn{1}{c|}{32006}  & \multicolumn{1}{c|}{0.17}  & \multicolumn{1}{c|}{30803}  & \multicolumn{1}{c|}{3.92}  & \multicolumn{1}{c|}{423}   & 4.73  \\
	                          & square                & \multicolumn{1}{c|}{18484}  & 250                          & \multicolumn{1}{c|}{18363}    & \multicolumn{1}{c|}{0.65}   & \multicolumn{1}{c|}{250}   & 0     & \multicolumn{1}{c|}{18302}  & \multicolumn{1}{c|}{0.98}  & \multicolumn{1}{c|}{250}   & 0    & \multicolumn{1}{c|}{15347}  & \multicolumn{1}{c|}{16.97} & \multicolumn{1}{c|}{18275}  & \multicolumn{1}{c|}{1.13}  & \multicolumn{1}{c|}{248}   & 0.80  \\
	                          & adder                 & \multicolumn{1}{c|}{1020}   & 255                          & \multicolumn{1}{c|}{1020}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{255}   & 0     & \multicolumn{1}{c|}{1019}   & \multicolumn{1}{c|}{0.10}  & \multicolumn{1}{c|}{255}   & 0    & \multicolumn{1}{c|}{1011}   & \multicolumn{1}{c|}{0.88}  & \multicolumn{1}{c|}{1019}   & \multicolumn{1}{c|}{0.10}  & \multicolumn{1}{c|}{255}   & 0     \\
	                          & sin                   & \multicolumn{1}{c|}{5416}   & 255                          & \multicolumn{1}{c|}{5337}     & \multicolumn{1}{c|}{1.46}   & \multicolumn{1}{c|}{223}   & 0.89  & \multicolumn{1}{c|}{5321}   & \multicolumn{1}{c|}{1.75}  & \multicolumn{1}{c|}{224}   & 0.44 & \multicolumn{1}{c|}{5404}   & \multicolumn{1}{c|}{0.22}  & \multicolumn{1}{c|}{5279}   & \multicolumn{1}{c|}{2.53}  & \multicolumn{1}{c|}{214}   & 4.89  \\
	                          & div                   & \multicolumn{1}{c|}{57235}  & 4372                         & \multicolumn{1}{c|}{41153}    & \multicolumn{1}{c|}{28.10}  & \multicolumn{1}{c|}{4372}  & 0     & \multicolumn{1}{c|}{56745}  & \multicolumn{1}{c|}{0.86}  & \multicolumn{1}{c|}{4372}  & 0    & \multicolumn{1}{c|}{57220}  & \multicolumn{1}{c|}{0.05}  & \multicolumn{1}{c|}{56550}  & \multicolumn{1}{c|}{1.20}  & \multicolumn{1}{c|}{4372}  & 0     \\
	                          & hyp                   & \multicolumn{1}{c|}{214335} & 24801                        & \multicolumn{1}{c|}{214274}   & \multicolumn{1}{c|}{0.03}   & \multicolumn{1}{c|}{24801} & 0     & \multicolumn{1}{c|}{212341} & \multicolumn{1}{c|}{0.93}  & \multicolumn{1}{c|}{24801} & 0    & \multicolumn{1}{c|}{196081} & \multicolumn{1}{c|}{8.52}  & \multicolumn{1}{c|}{212431} & \multicolumn{1}{c|}{0.89}  & \multicolumn{1}{c|}{24793} & 0.03  \\
	                          & max                   & \multicolumn{1}{c|}{2865}   & 287                          & \multicolumn{1}{c|}{2865}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{287}   & 0     & \multicolumn{1}{c|}{2865}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{287}   & 0    & \multicolumn{1}{c|}{2861}   & \multicolumn{1}{c|}{0.14}  & \multicolumn{1}{c|}{2865}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{214}   & 25.44 \\
	                          & sqrt                  & \multicolumn{1}{c|}{24617}  & 5058                         & \multicolumn{1}{c|}{19441}    & \multicolumn{1}{c|}{21.03}  & \multicolumn{1}{c|}{5058}  & 0     & \multicolumn{1}{c|}{23685}  & \multicolumn{1}{c|}{3.79}  & \multicolumn{1}{c|}{5058}  & 0    & \multicolumn{1}{c|}{24615}  & \multicolumn{1}{c|}{0.01}  & \multicolumn{1}{c|}{20155}  & \multicolumn{1}{c|}{18.13} & \multicolumn{1}{c|}{5056}  & 0.04  \\
	                          & multiplier            & \multicolumn{1}{c|}{27062}  & 274                          & \multicolumn{1}{c|}{26906}    & \multicolumn{1}{c|}{0.58}   & \multicolumn{1}{c|}{274}   & 0     & \multicolumn{1}{c|}{26814}  & \multicolumn{1}{c|}{0.92}  & \multicolumn{1}{c|}{274}   & 0    & \multicolumn{1}{c|}{26841}  & \multicolumn{1}{c|}{0.82}  & \multicolumn{1}{c|}{25509}  & \multicolumn{1}{c|}{5.74}  & \multicolumn{1}{c|}{272}   & 0.73  \\
	                          & bar                   & \multicolumn{1}{c|}{3336}   & 12                           & \multicolumn{1}{c|}{3141}     & \multicolumn{1}{c|}{5.85}   & \multicolumn{1}{c|}{12}    & 0     & \multicolumn{1}{c|}{3141}   & \multicolumn{1}{c|}{5.85}  & \multicolumn{1}{c|}{12}    & 0    & \multicolumn{1}{c|}{3142}   & \multicolumn{1}{c|}{5.82}  & \multicolumn{1}{c|}{3336}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{12}    & 0     \\ \hline
	\multirow{10}{*}{control} & priority              & \multicolumn{1}{c|}{978}    & 250                          & \multicolumn{1}{c|}{845}      & \multicolumn{1}{c|}{13.60}  & \multicolumn{1}{c|}{248}   & 0.80  & \multicolumn{1}{c|}{870}    & \multicolumn{1}{c|}{11.04} & \multicolumn{1}{c|}{227}   & 9.2  & \multicolumn{1}{c|}{970}    & \multicolumn{1}{c|}{0.82}  & \multicolumn{1}{c|}{888}    & \multicolumn{1}{c|}{9.20}  & \multicolumn{1}{c|}{242}   & 3.20  \\
	                          & cavlc                 & \multicolumn{1}{c|}{693}    & 16                           & \multicolumn{1}{c|}{691}      & \multicolumn{1}{c|}{0.29}   & \multicolumn{1}{c|}{16}    & 0     & \multicolumn{1}{c|}{690}    & \multicolumn{1}{c|}{0.43}  & \multicolumn{1}{c|}{16}    & 0    & \multicolumn{1}{c|}{679}    & \multicolumn{1}{c|}{2.02}  & \multicolumn{1}{c|}{688}    & \multicolumn{1}{c|}{0.72}  & \multicolumn{1}{c|}{16}    & 0     \\
	                          & arbiter               & \multicolumn{1}{c|}{11839}  & 87                           & \multicolumn{1}{c|}{11839}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{87}    & 0     & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{87}    & 0    & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{87}    & 0     \\
	                          & i2c                   & \multicolumn{1}{c|}{1342}   & 20                           & \multicolumn{1}{c|}{1311}     & \multicolumn{1}{c|}{2.31}   & \multicolumn{1}{c|}{20}    & 0     & \multicolumn{1}{c|}{1338}   & \multicolumn{1}{c|}{0.30}  & \multicolumn{1}{c|}{20}    & 0    & \multicolumn{1}{c|}{1316}   & \multicolumn{1}{c|}{1.94}  & \multicolumn{1}{c|}{1308}   & \multicolumn{1}{c|}{2.53}  & \multicolumn{1}{c|}{17}    & 15.00 \\
	                          & voter                 & \multicolumn{1}{c|}{13758}  & 70                           & \multicolumn{1}{c|}{11408}    & \multicolumn{1}{c|}{17.08}  & \multicolumn{1}{c|}{62}    & 11.43 & \multicolumn{1}{c|}{12681}  & \multicolumn{1}{c|}{7.83}  & \multicolumn{1}{c|}{63}    & 10   & \multicolumn{1}{c|}{12263}  & \multicolumn{1}{c|}{10.87} & \multicolumn{1}{c|}{11409}  & \multicolumn{1}{c|}{17.07} & \multicolumn{1}{c|}{70}    & 0     \\
	                          & int2float             & \multicolumn{1}{c|}{260}    & 16                           & \multicolumn{1}{c|}{225}      & \multicolumn{1}{c|}{13.46}  & \multicolumn{1}{c|}{15}    & 6.25  & \multicolumn{1}{c|}{251}    & \multicolumn{1}{c|}{3.46}  & \multicolumn{1}{c|}{16}    & 0    & \multicolumn{1}{c|}{222}    & \multicolumn{1}{c|}{14.62} & \multicolumn{1}{c|}{237}    & \multicolumn{1}{c|}{8.85}  & \multicolumn{1}{c|}{16}    & 0     \\
	                          & ctrl                  & \multicolumn{1}{c|}{174}    & 10                           & \multicolumn{1}{c|}{137}      & \multicolumn{1}{c|}{21.26}  & \multicolumn{1}{c|}{10}    & 0     & \multicolumn{1}{c|}{143}    & \multicolumn{1}{c|}{17.82} & \multicolumn{1}{c|}{9}     & 10   & \multicolumn{1}{c|}{131}    & \multicolumn{1}{c|}{24.71} & \multicolumn{1}{c|}{132}    & \multicolumn{1}{c|}{24.14} & \multicolumn{1}{c|}{9}     & 10.00 \\
	                          & dec                   & \multicolumn{1}{c|}{304}    & 3                            & \multicolumn{1}{c|}{304}      & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{3}     & 0     & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{3}     & 0    & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{3}     & 0     \\
	                          & mem\_ctrl             & \multicolumn{1}{c|}{46836}  & 114                          & \multicolumn{1}{c|}{46769}    & \multicolumn{1}{c|}{0.14}   & \multicolumn{1}{c|}{114}   & 0     & \multicolumn{1}{c|}{46582}  & \multicolumn{1}{c|}{0.54}  & \multicolumn{1}{c|}{114}   & 0    & \multicolumn{1}{c|}{46355}  & \multicolumn{1}{c|}{1.03}  & \multicolumn{1}{c|}{46076}  & \multicolumn{1}{c|}{1.62}  & \multicolumn{1}{c|}{113}   & 0.88  \\
	                          & router                & \multicolumn{1}{c|}{257}    & 54                           & \multicolumn{1}{c|}{254}      & \multicolumn{1}{c|}{1.17}   & \multicolumn{1}{c|}{52}    & 3.70  & \multicolumn{1}{c|}{246}    & \multicolumn{1}{c|}{4.28}  & \multicolumn{1}{c|}{54}    & 0    & \multicolumn{1}{c|}{247}    & \multicolumn{1}{c|}{3.89}  & \multicolumn{1}{c|}{242}    & \multicolumn{1}{c|}{5.84}  & \multicolumn{1}{c|}{28}    & 48.15 \\ \hline
	AVE                       &    -                   & \multicolumn{1}{c|}{}       &                              & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{6.43}   & \multicolumn{1}{c|}{}      & 1.16  & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{3.13}  & \multicolumn{1}{c|}{}      & 1.48 & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{4.675} & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{5.18}  & \multicolumn{1}{c|}{}      & 5.69  \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[thp]
\centering
\caption{Comparison the result of operators without preserving depth.}
\label{table:opt_not_preserve_depth}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|cc|cccc|cccc|cc|cccc|}
	\hline
	\multirow{2}{*}{}         & \multirow{2}{*}{name} & \multicolumn{2}{c|}{origin} & \multicolumn{4}{c|}{rewrite} & \multicolumn{4}{c|}{refactor} & \multicolumn{2}{c|}{date20} & \multicolumn{4}{c|}{ours}                                                                                                                                                                                                                                                                    \\ \cline{3-18}
	                          &                       & \multicolumn{1}{c|}{area}   & depth                        & \multicolumn{1}{c|}{area}     & \multicolumn{1}{c|}{a\%}    & \multicolumn{1}{c|}{depth} & d\%   & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{depth} & d\%  & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{depth} & d\%   \\ \hline
	\multirow{10}{*}{arith}   & log2                  & \multicolumn{1}{c|}{32060}  & 444                          & \multicolumn{1}{c|}{31547}    & \multicolumn{1}{c|}{1.60}   & \multicolumn{1}{c|}{443}   & 0.23  & \multicolumn{1}{c|}{31521}  & \multicolumn{1}{c|}{1.68}  & \multicolumn{1}{c|}{444}   & 0    & \multicolumn{1}{c|}{32006}  & \multicolumn{1}{c|}{0.17}  & \multicolumn{1}{c|}{30803}  & \multicolumn{1}{c|}{3.92}  & \multicolumn{1}{c|}{423}   & 4.73  \\
	                          & square                & \multicolumn{1}{c|}{18484}  & 250                          & \multicolumn{1}{c|}{18363}    & \multicolumn{1}{c|}{0.65}   & \multicolumn{1}{c|}{250}   & 0     & \multicolumn{1}{c|}{18302}  & \multicolumn{1}{c|}{0.98}  & \multicolumn{1}{c|}{250}   & 0    & \multicolumn{1}{c|}{15347}  & \multicolumn{1}{c|}{16.97} & \multicolumn{1}{c|}{18275}  & \multicolumn{1}{c|}{1.13}  & \multicolumn{1}{c|}{248}   & 0.80  \\
	                          & adder                 & \multicolumn{1}{c|}{1020}   & 255                          & \multicolumn{1}{c|}{1020}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{255}   & 0     & \multicolumn{1}{c|}{1019}   & \multicolumn{1}{c|}{0.10}  & \multicolumn{1}{c|}{255}   & 0    & \multicolumn{1}{c|}{1011}   & \multicolumn{1}{c|}{0.88}  & \multicolumn{1}{c|}{1019}   & \multicolumn{1}{c|}{0.10}  & \multicolumn{1}{c|}{255}   & 0     \\
	                          & sin                   & \multicolumn{1}{c|}{5416}   & 255                          & \multicolumn{1}{c|}{5337}     & \multicolumn{1}{c|}{1.46}   & \multicolumn{1}{c|}{223}   & 0.89  & \multicolumn{1}{c|}{5321}   & \multicolumn{1}{c|}{1.75}  & \multicolumn{1}{c|}{224}   & 0.44 & \multicolumn{1}{c|}{5404}   & \multicolumn{1}{c|}{0.22}  & \multicolumn{1}{c|}{5279}   & \multicolumn{1}{c|}{2.53}  & \multicolumn{1}{c|}{214}   & 4.89  \\
	                          & div                   & \multicolumn{1}{c|}{57235}  & 4372                         & \multicolumn{1}{c|}{41153}    & \multicolumn{1}{c|}{28.10}  & \multicolumn{1}{c|}{4372}  & 0     & \multicolumn{1}{c|}{56745}  & \multicolumn{1}{c|}{0.86}  & \multicolumn{1}{c|}{4372}  & 0    & \multicolumn{1}{c|}{57220}  & \multicolumn{1}{c|}{0.05}  & \multicolumn{1}{c|}{56550}  & \multicolumn{1}{c|}{1.20}  & \multicolumn{1}{c|}{4372}  & 0     \\
	                          & hyp                   & \multicolumn{1}{c|}{214335} & 24801                        & \multicolumn{1}{c|}{214274}   & \multicolumn{1}{c|}{0.03}   & \multicolumn{1}{c|}{24801} & 0     & \multicolumn{1}{c|}{212341} & \multicolumn{1}{c|}{0.93}  & \multicolumn{1}{c|}{24801} & 0    & \multicolumn{1}{c|}{196081} & \multicolumn{1}{c|}{8.52}  & \multicolumn{1}{c|}{212431} & \multicolumn{1}{c|}{0.89}  & \multicolumn{1}{c|}{24793} & 0.03  \\
	                          & max                   & \multicolumn{1}{c|}{2865}   & 287                          & \multicolumn{1}{c|}{2865}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{287}   & 0     & \multicolumn{1}{c|}{2865}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{287}   & 0    & \multicolumn{1}{c|}{2861}   & \multicolumn{1}{c|}{0.14}  & \multicolumn{1}{c|}{2865}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{214}   & 25.44 \\
	                          & sqrt                  & \multicolumn{1}{c|}{24617}  & 5058                         & \multicolumn{1}{c|}{19441}    & \multicolumn{1}{c|}{21.03}  & \multicolumn{1}{c|}{5058}  & 0     & \multicolumn{1}{c|}{23685}  & \multicolumn{1}{c|}{3.79}  & \multicolumn{1}{c|}{5058}  & 0    & \multicolumn{1}{c|}{24615}  & \multicolumn{1}{c|}{0.01}  & \multicolumn{1}{c|}{20155}  & \multicolumn{1}{c|}{18.13} & \multicolumn{1}{c|}{5056}  & 0.04  \\
	                          & multiplier            & \multicolumn{1}{c|}{27062}  & 274                          & \multicolumn{1}{c|}{26906}    & \multicolumn{1}{c|}{0.58}   & \multicolumn{1}{c|}{274}   & 0     & \multicolumn{1}{c|}{26814}  & \multicolumn{1}{c|}{0.92}  & \multicolumn{1}{c|}{274}   & 0    & \multicolumn{1}{c|}{26841}  & \multicolumn{1}{c|}{0.82}  & \multicolumn{1}{c|}{25509}  & \multicolumn{1}{c|}{5.74}  & \multicolumn{1}{c|}{272}   & 0.73  \\
	                          & bar                   & \multicolumn{1}{c|}{3336}   & 12                           & \multicolumn{1}{c|}{3141}     & \multicolumn{1}{c|}{5.85}   & \multicolumn{1}{c|}{12}    & 0     & \multicolumn{1}{c|}{3141}   & \multicolumn{1}{c|}{5.85}  & \multicolumn{1}{c|}{12}    & 0    & \multicolumn{1}{c|}{3142}   & \multicolumn{1}{c|}{5.82}  & \multicolumn{1}{c|}{3336}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{12}    & 0     \\ \hline
	\multirow{10}{*}{control} & priority              & \multicolumn{1}{c|}{978}    & 250                          & \multicolumn{1}{c|}{845}      & \multicolumn{1}{c|}{13.60}  & \multicolumn{1}{c|}{248}   & 0.80  & \multicolumn{1}{c|}{870}    & \multicolumn{1}{c|}{11.04} & \multicolumn{1}{c|}{227}   & 9.2  & \multicolumn{1}{c|}{970}    & \multicolumn{1}{c|}{0.82}  & \multicolumn{1}{c|}{888}    & \multicolumn{1}{c|}{9.20}  & \multicolumn{1}{c|}{242}   & 3.20  \\
	                          & cavlc                 & \multicolumn{1}{c|}{693}    & 16                           & \multicolumn{1}{c|}{691}      & \multicolumn{1}{c|}{0.29}   & \multicolumn{1}{c|}{16}    & 0     & \multicolumn{1}{c|}{690}    & \multicolumn{1}{c|}{0.43}  & \multicolumn{1}{c|}{16}    & 0    & \multicolumn{1}{c|}{679}    & \multicolumn{1}{c|}{2.02}  & \multicolumn{1}{c|}{688}    & \multicolumn{1}{c|}{0.72}  & \multicolumn{1}{c|}{16}    & 0     \\
	                          & arbiter               & \multicolumn{1}{c|}{11839}  & 87                           & \multicolumn{1}{c|}{11839}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{87}    & 0     & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{87}    & 0    & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{87}    & 0     \\
	                          & i2c                   & \multicolumn{1}{c|}{1342}   & 20                           & \multicolumn{1}{c|}{1311}     & \multicolumn{1}{c|}{2.31}   & \multicolumn{1}{c|}{20}    & 0     & \multicolumn{1}{c|}{1338}   & \multicolumn{1}{c|}{0.30}  & \multicolumn{1}{c|}{20}    & 0    & \multicolumn{1}{c|}{1316}   & \multicolumn{1}{c|}{1.94}  & \multicolumn{1}{c|}{1308}   & \multicolumn{1}{c|}{2.53}  & \multicolumn{1}{c|}{17}    & 15.00 \\
	                          & voter                 & \multicolumn{1}{c|}{13758}  & 70                           & \multicolumn{1}{c|}{11408}    & \multicolumn{1}{c|}{17.08}  & \multicolumn{1}{c|}{62}    & 11.43 & \multicolumn{1}{c|}{12681}  & \multicolumn{1}{c|}{7.83}  & \multicolumn{1}{c|}{63}    & 10   & \multicolumn{1}{c|}{12263}  & \multicolumn{1}{c|}{10.87} & \multicolumn{1}{c|}{11409}  & \multicolumn{1}{c|}{17.07} & \multicolumn{1}{c|}{70}    & 0     \\
	                          & int2float             & \multicolumn{1}{c|}{260}    & 16                           & \multicolumn{1}{c|}{225}      & \multicolumn{1}{c|}{13.46}  & \multicolumn{1}{c|}{15}    & 6.25  & \multicolumn{1}{c|}{251}    & \multicolumn{1}{c|}{3.46}  & \multicolumn{1}{c|}{16}    & 0    & \multicolumn{1}{c|}{222}    & \multicolumn{1}{c|}{14.62} & \multicolumn{1}{c|}{237}    & \multicolumn{1}{c|}{8.85}  & \multicolumn{1}{c|}{16}    & 0     \\
	                          & ctrl                  & \multicolumn{1}{c|}{174}    & 10                           & \multicolumn{1}{c|}{137}      & \multicolumn{1}{c|}{21.26}  & \multicolumn{1}{c|}{10}    & 0     & \multicolumn{1}{c|}{143}    & \multicolumn{1}{c|}{17.82} & \multicolumn{1}{c|}{9}     & 10   & \multicolumn{1}{c|}{131}    & \multicolumn{1}{c|}{24.71} & \multicolumn{1}{c|}{132}    & \multicolumn{1}{c|}{24.14} & \multicolumn{1}{c|}{9}     & 10.00 \\
	                          & dec                   & \multicolumn{1}{c|}{304}    & 3                            & \multicolumn{1}{c|}{304}      & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{3}     & 0     & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{3}     & 0    & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{3}     & 0     \\
	                          & mem\_ctrl             & \multicolumn{1}{c|}{46836}  & 114                          & \multicolumn{1}{c|}{46769}    & \multicolumn{1}{c|}{0.14}   & \multicolumn{1}{c|}{114}   & 0     & \multicolumn{1}{c|}{46582}  & \multicolumn{1}{c|}{0.54}  & \multicolumn{1}{c|}{114}   & 0    & \multicolumn{1}{c|}{46355}  & \multicolumn{1}{c|}{1.03}  & \multicolumn{1}{c|}{46076}  & \multicolumn{1}{c|}{1.62}  & \multicolumn{1}{c|}{113}   & 0.88  \\
	                          & router                & \multicolumn{1}{c|}{257}    & 54                           & \multicolumn{1}{c|}{254}      & \multicolumn{1}{c|}{1.17}   & \multicolumn{1}{c|}{52}    & 3.70  & \multicolumn{1}{c|}{246}    & \multicolumn{1}{c|}{4.28}  & \multicolumn{1}{c|}{54}    & 0    & \multicolumn{1}{c|}{247}    & \multicolumn{1}{c|}{3.89}  & \multicolumn{1}{c|}{242}    & \multicolumn{1}{c|}{5.84}  & \multicolumn{1}{c|}{28}    & 48.15 \\ \hline
	AVE                       &                       & \multicolumn{1}{c|}{}       &                              & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{6.43}   & \multicolumn{1}{c|}{}      & 1.16  & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{3.13}  & \multicolumn{1}{c|}{}      & 1.48 & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{4.675} & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{5.18}  & \multicolumn{1}{c|}{}      & 5.69  \\ \hline
\end{tabular}
}
\end{table*}

\subsection{Evaluation of scalability}

\subsubsection{balance-aware的消融实验}
\subsubsection{Result of multiple operators}

focus on the sequential optimization with other optimizer, like resyn or resyn2
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[thp]
	\centering
	\caption{Result of post-optimization for $resyn$ and $resyn2$.}
 \resizebox{\linewidth}{!}{
	\begin{tabular}{|c|c|cc|cccc|cccc|cccc|}
		\hline
		\multirow{2}{*}{}         & \multirow{2}{*}{name} & \multicolumn{2}{c|}{origin} & \multicolumn{4}{c|}{resyn} & \multicolumn{4}{c|}{resyn2} & \multicolumn{4}{c|}{ours}                                                                                                                                                                                                                                       \\ \cline{3-16}
		                          &                       & \multicolumn{1}{c|}{area}   & depth                      & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{depth} & d\%   & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{depth} & d\%   & \multicolumn{1}{c|}{area}   & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{depth} & d\%   \\ \hline
		\multirow{10}{*}{arith}   & log2                  & \multicolumn{1}{c|}{32060}  & 444                        & \multicolumn{1}{c|}{30231}  & \multicolumn{1}{c|}{5.70}  & \multicolumn{1}{c|}{382}   & 13.96 & \multicolumn{1}{c|}{29370}  & \multicolumn{1}{c|}{8.39}  & \multicolumn{1}{c|}{376}   & 15.32 & \multicolumn{1}{c|}{29257}  & \multicolumn{1}{c|}{8.74}  & \multicolumn{1}{c|}{376}   & 15.32 \\
		                          & square                & \multicolumn{1}{c|}{18484}  & 250                        & \multicolumn{1}{c|}{16914}  & \multicolumn{1}{c|}{8.49}  & \multicolumn{1}{c|}{248}   & 0.80  & \multicolumn{1}{c|}{16623}  & \multicolumn{1}{c|}{10.07} & \multicolumn{1}{c|}{248}   & 0.80  & \multicolumn{1}{c|}{16662}  & \multicolumn{1}{c|}{9.86}  & \multicolumn{1}{c|}{248}   & 0.80  \\
		                          & adder                 & \multicolumn{1}{c|}{1020}   & 255                        & \multicolumn{1}{c|}{1020}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{255}   & 0     & \multicolumn{1}{c|}{1019}   & \multicolumn{1}{c|}{0.10}  & \multicolumn{1}{c|}{255}   & 0     & \multicolumn{1}{c|}{1019}   & \multicolumn{1}{c|}{0.10}  & \multicolumn{1}{c|}{255}   & 0     \\
		                          & sin                   & \multicolumn{1}{c|}{5416}   & 225                        & \multicolumn{1}{c|}{5132}   & \multicolumn{1}{c|}{5.24}  & \multicolumn{1}{c|}{179}   & 20.44 & \multicolumn{1}{c|}{5039}   & \multicolumn{1}{c|}{6.96}  & \multicolumn{1}{c|}{177}   & 21.33 & \multicolumn{1}{c|}{5043}   & \multicolumn{1}{c|}{6.89}  & \multicolumn{1}{c|}{172}   & 23.56 \\
		                          & div                   & \multicolumn{1}{c|}{57235}  & 4372                       & \multicolumn{1}{c|}{40889}  & \multicolumn{1}{c|}{28.56} & \multicolumn{1}{c|}{4359}  & 0.30  & \multicolumn{1}{c|}{40772}  & \multicolumn{1}{c|}{28.76} & \multicolumn{1}{c|}{4361}  & 0.25  & \multicolumn{1}{c|}{40751}  & \multicolumn{1}{c|}{28.80} & \multicolumn{1}{c|}{4364}  & 0.18  \\
		                          & hyp                   & \multicolumn{1}{c|}{214335} & 24801                      & \multicolumn{1}{c|}{214240} & \multicolumn{1}{c|}{0.04}  & \multicolumn{1}{c|}{24802} & 0     & \multicolumn{1}{c|}{211330} & \multicolumn{1}{c|}{1.40}  & \multicolumn{1}{c|}{24794} & 0.03  & \multicolumn{1}{c|}{211536} & \multicolumn{1}{c|}{1.31}  & \multicolumn{1}{c|}{24786} & 0.06  \\
		                          & max                   & \multicolumn{1}{c|}{2865}   & 287                        & \multicolumn{1}{c|}{2861}   & \multicolumn{1}{c|}{0.14}  & \multicolumn{1}{c|}{217}   & 24.39 & \multicolumn{1}{c|}{2834}   & \multicolumn{1}{c|}{1.08}  & \multicolumn{1}{c|}{204}   & 28.92 & \multicolumn{1}{c|}{2858}   & \multicolumn{1}{c|}{0.24}  & \multicolumn{1}{c|}{179}   & 37.63 \\
		                          & sqrt                  & \multicolumn{1}{c|}{24617}  & 5058                       & \multicolumn{1}{c|}{19437}  & \multicolumn{1}{c|}{21.04} & \multicolumn{1}{c|}{5058}  & 0     & \multicolumn{1}{c|}{19437}  & \multicolumn{1}{c|}{21.04} & \multicolumn{1}{c|}{4968}  & 1.78  & \multicolumn{1}{c|}{19439}  & \multicolumn{1}{c|}{21.03} & \multicolumn{1}{c|}{4975}  & 1.64  \\
		                          & multiplier            & \multicolumn{1}{c|}{27062}  & 274                        & \multicolumn{1}{c|}{25200}  & \multicolumn{1}{c|}{6.88}  & \multicolumn{1}{c|}{263}   & 4.01  & \multicolumn{1}{c|}{24556}  & \multicolumn{1}{c|}{9.26}  & \multicolumn{1}{c|}{262}   & 4.38  & \multicolumn{1}{c|}{24379}  & \multicolumn{1}{c|}{9.91}  & \multicolumn{1}{c|}{262}   & 4.38  \\
		                          & bar                   & \multicolumn{1}{c|}{3336}   & 12                         & \multicolumn{1}{c|}{3141}   & \multicolumn{1}{c|}{5.85}  & \multicolumn{1}{c|}{12}    & 0     & \multicolumn{1}{c|}{3141}   & \multicolumn{1}{c|}{5.85}  & \multicolumn{1}{c|}{12}    & 0     & \multicolumn{1}{c|}{3141}   & \multicolumn{1}{c|}{5.85}  & \multicolumn{1}{c|}{12}    & 0     \\ \hline
		\multirow{10}{*}{control} & priority              & \multicolumn{1}{c|}{978}    & 250                        & \multicolumn{1}{c|}{810}    & \multicolumn{1}{c|}{17.18} & \multicolumn{1}{c|}{240}   & 4.00  & \multicolumn{1}{c|}{676}    & \multicolumn{1}{c|}{30.88} & \multicolumn{1}{c|}{203}   & 18.80 & \multicolumn{1}{c|}{764}    & \multicolumn{1}{c|}{21.88} & \multicolumn{1}{c|}{232}   & 7.20  \\
		                          & cavlc                 & \multicolumn{1}{c|}{693}    & 16                         & \multicolumn{1}{c|}{673}    & \multicolumn{1}{c|}{2.89}  & \multicolumn{1}{c|}{16}    & 0     & \multicolumn{1}{c|}{662}    & \multicolumn{1}{c|}{4.47}  & \multicolumn{1}{c|}{16}    & 0     & \multicolumn{1}{c|}{659}    & \multicolumn{1}{c|}{4.91}  & \multicolumn{1}{c|}{16}    & 0     \\
		                          & arbiter               & \multicolumn{1}{c|}{11839}  & 87                         & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{87}    & 0     & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{87}    & 0     & \multicolumn{1}{c|}{11839}  & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{87}    & 0     \\
		                          & i2c                   & \multicolumn{1}{c|}{1342}   & 20                         & \multicolumn{1}{c|}{1185}   & \multicolumn{1}{c|}{11.70} & \multicolumn{1}{c|}{16}    & 20.00 & \multicolumn{1}{c|}{1162}   & \multicolumn{1}{c|}{13.41} & \multicolumn{1}{c|}{15}    & 25.00 & \multicolumn{1}{c|}{1143}   & \multicolumn{1}{c|}{14.83} & \multicolumn{1}{c|}{16}    & 20.00 \\
		                          & voter                 & \multicolumn{1}{c|}{13758}  & 70                         & \multicolumn{1}{c|}{10455}  & \multicolumn{1}{c|}{24.01} & \multicolumn{1}{c|}{59}    & 15.71 & \multicolumn{1}{c|}{9756}   & \multicolumn{1}{c|}{29.09} & \multicolumn{1}{c|}{57}    & 18.57 & \multicolumn{1}{c|}{8743}   & \multicolumn{1}{c|}{36.45} & \multicolumn{1}{c|}{58}    & 17.14 \\
		                          & int2float             & \multicolumn{1}{c|}{260}    & 16                         & \multicolumn{1}{c|}{217}    & \multicolumn{1}{c|}{16.54} & \multicolumn{1}{c|}{15}    & 6.25  & \multicolumn{1}{c|}{214}    & \multicolumn{1}{c|}{17.69} & \multicolumn{1}{c|}{15}    & 6.25  & \multicolumn{1}{c|}{210}    & \multicolumn{1}{c|}{19.23} & \multicolumn{1}{c|}{15}    & 6.25  \\
		                          & ctrl                  & \multicolumn{1}{c|}{174}    & 10                         & \multicolumn{1}{c|}{124}    & \multicolumn{1}{c|}{28.74} & \multicolumn{1}{c|}{10}    & 0     & \multicolumn{1}{c|}{108}    & \multicolumn{1}{c|}{37.93} & \multicolumn{1}{c|}{8}     & 20.00 & \multicolumn{1}{c|}{107}    & \multicolumn{1}{c|}{38.51} & \multicolumn{1}{c|}{8}     & 20.00 \\
		                          & dec                   & \multicolumn{1}{c|}{304}    & 3                          & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{3}     & 0     & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{3}     & 0     & \multicolumn{1}{c|}{304}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{3}     & 0     \\
		                          & mem\_ctrl              & \multicolumn{1}{c|}{46836}  & 114                        & \multicolumn{1}{c|}{46613}  & \multicolumn{1}{c|}{0.48}  & \multicolumn{1}{c|}{112}   & 1.75  & \multicolumn{1}{c|}{45614}  & \multicolumn{1}{c|}{2.61}  & \multicolumn{1}{c|}{110}   & 3.51  & \multicolumn{1}{c|}{44949}  & \multicolumn{1}{c|}{4.03}  & \multicolumn{1}{c|}{107}   & 6.14  \\
		                          & router                & \multicolumn{1}{c|}{257}    & 54                         & \multicolumn{1}{c|}{241}    & \multicolumn{1}{c|}{6.23}  & \multicolumn{1}{c|}{26}    & 51.85 & \multicolumn{1}{c|}{177}    & \multicolumn{1}{c|}{31.13} & \multicolumn{1}{c|}{19}    & 64.81 & \multicolumn{1}{c|}{202}    & \multicolumn{1}{c|}{21.40} & \multicolumn{1}{c|}{23}    & 57.41 \\ \hline
		AVE                       &                       & \multicolumn{1}{c|}{}       &                            & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{9.49}  & \multicolumn{1}{c|}{}      & 8.17  & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{13.01} & \multicolumn{1}{c|}{}      & 11.49 & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{12.70} & \multicolumn{1}{c|}{}      & 10.89 \\ \hline
	\end{tabular}
 }
\end{table*}

% \subsection{Result of technology mapping}
% focus on the technology mapping result on result AIG file.
% write the scripts for the dchoice

% {\color{red}result of mapping is not good, and how to say scalability?}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[thp]
% 	\centering
% 	\caption{result of technology mapping}
%  \resizebox{\linewidth}{!}{
% 	\begin{tabular}{|c|c|cc|cccc|cccccccc|}
% 		\hline
% 		\multirow{3}{*}{type}     & \multirow{3}{*}{name} & \multicolumn{2}{c|}{origin}                & \multicolumn{4}{c|}{dchoice} & \multicolumn{8}{c|}{dchoice+ours}                                                                                                                                                                                                                                                                                                                        \\ \cline{3-16}
% 		                          &                       & \multicolumn{1}{c|}{\multirow{2}{*}{area}} & \multirow{2}{*}{depth}       & \multicolumn{2}{c|}{FPGA}         & \multicolumn{2}{c|}{ASIC}  & \multicolumn{4}{c|}{FPGA}      & \multicolumn{4}{c|}{ASIC}                                                                                                                                                                                                                              \\ \cline{5-16}
% 		                          &                       & \multicolumn{1}{c|}{}                      &                              & \multicolumn{1}{c|}{area}         & \multicolumn{1}{c|}{delay} & \multicolumn{1}{c|}{area}      & delay                     & \multicolumn{1}{c|}{area}  & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{delay} & \multicolumn{1}{c|}{d\%}    & \multicolumn{1}{c|}{area}      & \multicolumn{1}{c|}{a\%}   & \multicolumn{1}{c|}{delay}     & d\%    \\ \hline
% 		\multirow{10}{*}{arith}   & log2                  & \multicolumn{1}{c|}{32060}                 & 444                          & \multicolumn{1}{c|}{8270}         & \multicolumn{1}{c|}{67}    & \multicolumn{1}{c|}{29146.17}  & 3379.98                   & \multicolumn{1}{c|}{8125}  & \multicolumn{1}{c|}{1.75}  & \multicolumn{1}{c|}{66}    & \multicolumn{1}{c|}{1.49}   & \multicolumn{1}{c|}{30300.86}  & \multicolumn{1}{c|}{-3.96} & \multicolumn{1}{c|}{3119.45}   & 7.71   \\
% 		                          & square                & \multicolumn{1}{c|}{18484}                 & 250                          & \multicolumn{1}{c|}{4255}         & \multicolumn{1}{c|}{50}    & \multicolumn{1}{c|}{16161.01}  & 1785.42                   & \multicolumn{1}{c|}{4213}  & \multicolumn{1}{c|}{0.99}  & \multicolumn{1}{c|}{50}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{16485.24}  & \multicolumn{1}{c|}{-2.01} & \multicolumn{1}{c|}{1770.11}   & 0.86   \\
% 		                          & adder                 & \multicolumn{1}{c|}{1020}                  & 255                          & \multicolumn{1}{c|}{273}          & \multicolumn{1}{c|}{51}    & \multicolumn{1}{c|}{1213.79}   & 1805.76                   & \multicolumn{1}{c|}{272}   & \multicolumn{1}{c|}{0.37}  & \multicolumn{1}{c|}{51}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{1187.6}    & \multicolumn{1}{c|}{2.16}  & \multicolumn{1}{c|}{1805.76}   & 0      \\
% 		                          & sin                   & \multicolumn{1}{c|}{5416}                  & 225                          & \multicolumn{1}{c|}{1473}         & \multicolumn{1}{c|}{35}    & \multicolumn{1}{c|}{6130.84}   & 1546.26                   & \multicolumn{1}{c|}{1491}  & \multicolumn{1}{c|}{-1.22} & \multicolumn{1}{c|}{36}    & \multicolumn{1}{c|}{-2.86}  & \multicolumn{1}{c|}{5774.38}   & \multicolumn{1}{c|}{5.81}  & \multicolumn{1}{c|}{1605.26}   & -3.82  \\
% 		                          & div                   & \multicolumn{1}{c|}{57235}                 & 4372                         & \multicolumn{1}{c|}{7326}         & \multicolumn{1}{c|}{857}   & \multicolumn{1}{c|}{31930.41}  & 43322.5                   & \multicolumn{1}{c|}{7638}  & \multicolumn{1}{c|}{-4.26} & \multicolumn{1}{c|}{858}   & \multicolumn{1}{c|}{-0.12}  & \multicolumn{1}{c|}{33728.81}  & \multicolumn{1}{c|}{-5.63} & \multicolumn{1}{c|}{43146.42}  & 0.41   \\
% 		                          & hyp                   & \multicolumn{1}{c|}{214335}                & 24801                        & \multicolumn{1}{c|}{46427}        & \multicolumn{1}{c|}{4173}  & \multicolumn{1}{c|}{213140.73} & 174284.69                 & \multicolumn{1}{c|}{47371} & \multicolumn{1}{c|}{-2.03} & \multicolumn{1}{c|}{4193}  & \multicolumn{1}{c|}{-0.48}  & \multicolumn{1}{c|}{208872.75} & \multicolumn{1}{c|}{2.00}  & \multicolumn{1}{c|}{175053.06} & -0.44  \\
% 		                          & max                   & \multicolumn{1}{c|}{2865}                  & 287                          & \multicolumn{1}{c|}{820}          & \multicolumn{1}{c|}{34}    & \multicolumn{1}{c|}{2463.24}   & 1608.93                   & \multicolumn{1}{c|}{832}   & \multicolumn{1}{c|}{-1.46} & \multicolumn{1}{c|}{34}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{2489.66}   & \multicolumn{1}{c|}{-1.07} & \multicolumn{1}{c|}{1707.38}   & -6.12  \\
% 		                          & sqrt                  & \multicolumn{1}{c|}{24617}                 & 5058                         & \multicolumn{1}{c|}{5071}         & \multicolumn{1}{c|}{990}   & \multicolumn{1}{c|}{22694.49}  & 47397.75                  & \multicolumn{1}{c|}{4300}  & \multicolumn{1}{c|}{15.20} & \multicolumn{1}{c|}{1002}  & \multicolumn{1}{c|}{-1.21}  & \multicolumn{1}{c|}{21805.83}  & \multicolumn{1}{c|}{3.92}  & \multicolumn{1}{c|}{47716.04}  & -0.67  \\
% 		                          & multiplier            & \multicolumn{1}{c|}{27062}                 & 274                          & \multicolumn{1}{c|}{6090}         & \multicolumn{1}{c|}{53}    & \multicolumn{1}{c|}{24681.92}  & 2672.99                   & \multicolumn{1}{c|}{6025}  & \multicolumn{1}{c|}{1.07}  & \multicolumn{1}{c|}{53}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{22230.04}  & \multicolumn{1}{c|}{9.93}  & \multicolumn{1}{c|}{2674.27}   & -0.05  \\
% 		                          & bar                   & \multicolumn{1}{c|}{3336}                  & 12                           & \multicolumn{1}{c|}{512}          & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{2507.86}   & 147.44                    & \multicolumn{1}{c|}{512}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{2621.58}   & \multicolumn{1}{c|}{-4.53} & \multicolumn{1}{c|}{149.88}    & -1.65  \\ \hline
% 		\multirow{10}{*}{control} & priority              & \multicolumn{1}{c|}{978}                   & 250                          & \multicolumn{1}{c|}{183}          & \multicolumn{1}{c|}{27}    & \multicolumn{1}{c|}{812.11}    & 1451.23                   & \multicolumn{1}{c|}{192}   & \multicolumn{1}{c|}{-4.92} & \multicolumn{1}{c|}{29}    & \multicolumn{1}{c|}{-7.41}  & \multicolumn{1}{c|}{871.62}    & \multicolumn{1}{c|}{-7.33} & \multicolumn{1}{c|}{1572.59}   & -8.36  \\
% 		                          & cavlc                 & \multicolumn{1}{c|}{693}                   & 16                           & \multicolumn{1}{c|}{116}          & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{453.18}    & 150.66                    & \multicolumn{1}{c|}{118}   & \multicolumn{1}{c|}{-1.72} & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{434.22}    & \multicolumn{1}{c|}{4.18}  & \multicolumn{1}{c|}{169.59}    & -12.56 \\
% 		                          & arbiter               & \multicolumn{1}{c|}{11839}                 & 87                           & \multicolumn{1}{c|}{2722}         & \multicolumn{1}{c|}{18}    & \multicolumn{1}{c|}{7678.93}   & 906.64                    & \multicolumn{1}{c|}{2721}  & \multicolumn{1}{c|}{0.04}  & \multicolumn{1}{c|}{18}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{7679.16}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{906.64}    & 0      \\
% 		                          & i2c                   & \multicolumn{1}{c|}{1342}                  & 20                           & \multicolumn{1}{c|}{340}          & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{778.33}    & 132.76                    & \multicolumn{1}{c|}{324}   & \multicolumn{1}{c|}{4.71}  & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{769.3}     & \multicolumn{1}{c|}{1.16}  & \multicolumn{1}{c|}{131.69}    & 0.81   \\
% 		                          & voter                 & \multicolumn{1}{c|}{13758}                 & 70                           & \multicolumn{1}{c|}{1505}         & \multicolumn{1}{c|}{12}    & \multicolumn{1}{c|}{17673.41}  & 577.79                    & \multicolumn{1}{c|}{1631}  & \multicolumn{1}{c|}{-8.37} & \multicolumn{1}{c|}{12}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{13515.8}   & \multicolumn{1}{c|}{23.52} & \multicolumn{1}{c|}{603.64}    & -4.47  \\
% 		                          & int2float             & \multicolumn{1}{c|}{260}                   & 16                           & \multicolumn{1}{c|}{47}           & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{146}       & 116.9                     & \multicolumn{1}{c|}{46}    & \multicolumn{1}{c|}{2.13}  & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{140.15}    & \multicolumn{1}{c|}{4.01}  & \multicolumn{1}{c|}{122.22}    & -4.55  \\
% 		                          & ctrl                  & \multicolumn{1}{c|}{174}                   & 10                           & \multicolumn{1}{c|}{29}           & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{80.96}     & 74.4                      & \multicolumn{1}{c|}{29}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{76.77}     & \multicolumn{1}{c|}{5.18}  & \multicolumn{1}{c|}{75.77}     & -1.84  \\
% 		                          & dec                   & \multicolumn{1}{c|}{304}                   & 3                            & \multicolumn{1}{c|}{287}          & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{289.42}    & 54.39                     & \multicolumn{1}{c|}{287}   & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{289.42}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{54.39}     & 0      \\
% 		                          & mem\_ctrl             & \multicolumn{1}{c|}{46836}                 & 114                          & \multicolumn{1}{c|}{11541}        & \multicolumn{1}{c|}{20}    & \multicolumn{1}{c|}{28971.04}  & 792.75                    & \multicolumn{1}{c|}{11620} & \multicolumn{1}{c|}{-0.68} & \multicolumn{1}{c|}{22}    & \multicolumn{1}{c|}{-10.00} & \multicolumn{1}{c|}{29528.9}   & \multicolumn{1}{c|}{-1.93} & \multicolumn{1}{c|}{860.08}    & -8.49  \\
% 		                          & router                & \multicolumn{1}{c|}{257}                   & 54                           & \multicolumn{1}{c|}{92}           & \multicolumn{1}{c|}{6}     & \multicolumn{1}{c|}{222.34}    & 221.59                    & \multicolumn{1}{c|}{84}    & \multicolumn{1}{c|}{8.70}  & \multicolumn{1}{c|}{6}     & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{199.19}    & \multicolumn{1}{c|}{10.41} & \multicolumn{1}{c|}{208.95}    & 5.70   \\ \hline
% 		AVE                       &                       & \multicolumn{1}{c|}{}                      &                              & \multicolumn{1}{c|}{}             & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}          &                           & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{0.51}  & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{-1.03}  & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{2.29}  & \multicolumn{1}{c|}{}          & -1.88  \\ \hline
% 	\end{tabular}
%  }
% \end{table*}

% \subsection{Analysis of parallelism}
% Just Analysis?!
% focus on the parallel analysis, it will do not break the attribute of parallelism. \\
% 1. Level-constrained parallelism to maintain the QoR; \\
% 2. random parallelism to lift speed.

\subsection{Discussion}

==> sections/introduction.tex <==
\section{introduction}
\label{sec:intro}
Logic level optimization\cite{synthesis} is an essential step to reduce the area and depth for a circuit to meet a better performance, power and area~(PPA).
Rewriting is a highly flexible and efficient technique for logic level optimization, making it a frequently employed method to achieve circuit area or depth reduction.
The primary objective of rewriting is to substitute a subgraph in a circuit with another subgraph that has lower cost but equivalent functionality.

In the era of two-level logic, rewriting is achieved through two steps due to the specific structure of circuits: Boolean algebra~(also known as Boolean expression) optimization and their subsequent replacement.
Espresso\cite{two-level} is a typical tool for Boolean algebra optimization during that period.
With the development of Very large-scale integration~(VLSI) technology, multi-level logic has emerged as a crucial component in logic synthesis.
And in the era of multi-level logic, the circuits are depicted as Boolean networks comprising logic gates. Therefore, graph-based manipulation techniques [3] have emerged as the predominant methods by leveraging the structure properties of these networks.
Specifically,  the rewriting methods based on graph manipulation comprises primarily of the following four steps:
\begin{itemize}
    \item \textbf{Cone computation}. A Maximum Fanout Free Cone~(\textit{MFFC}) of a node $n$ is a multi-input sub-circuit where each path from a node in this sub-circuit to any outputs of the whole circuit passes through $n$.
    The underlying principle of rewriting based on MFFC is that the internal nodes have no external dependencies and can be replaced equivalently even though we change its structure.
    \item \textbf{MFFC optimization}. As MFFC is a multi-input and single-output Boolean graph, there exist various optimization methods available for it, such as pattern rewriting and Boolean algebra minimization based on the corresponding cost function.
    \item \textbf{Cost evaluation}. After the MFFC optimization step, it is necessary to evaluate the cost when replacing the original MFFC with the newly optimized one in order to achieve better quality. The cost may include area, depth, edges, etc.
    \item \textbf{Equivalent replacement}. The inputs and outputs of the newly optimized subgraph resulting from MFFC optimization may be permuted or negated in comparison to the original MFFC. Therefore, this step ensures correct connectivity relations and equivalence.
\end{itemize}

There are various techniques available to accomplish the rewriting process at different scales. 
{\color{red}通过方法进行分类.}
Darringer \textit{et.al} proposed the pattern-based rewriting\cite{pattern-rewrite}, it is based on the rule-based local transformation, the patterns need to be collected already.
Its problem is that the patterns' space is exponential with the input size grow.
The irredundant SOP~(iSOP) \cite{isop}-based Boolean algebra minimization has beeen applied in many methods\cite{large-SOP-opt}\cite{brayton2006scalable}. It mainly remove the sharing literals or clauses to reduce the cost. It is efficient when the input size is large, but it may get stuck in local optimal due to worst iSOP.
The NPN~(Negate, Permute, Negate) classification\cite{NPN-class} for Boolean function is commonly used in rewriting.
It expands the equivalent structures' search space by adding the process for negating inputs, permuting inputs or negating output of a Boolean function.
Alan \textit{et.al} has implemented the 4-input NPN-based rewriting\cite{NPN-rewrite-4} method through 4-feasible-cut enumeration in ABC\cite{berkeley-abc} tool.
However, it is hard to expand beyond 4-input.
Li \textit{et.al}\cite{NPN-rewrite-5} has just extended the 4-input NPN-based rewriting to 5-input by partial NPN classes.
Heinz \textit{et.al} proposed an exact way to implement rewriting with optimal local area replacement.
The on-the fly exact synthesis\cite{exact-rw-date19} suffers from the time cost by solving the optimal local area/delay through incrementally SAT-based encoding and checking for Boolean functions\cite{exact-synthesis-TCAD20}. 
And also the exact rewriting\cite{exact-rw-date20} is still within the framework of $k$-input NPN-based rewriting.

All these rewriting algorithms above only has its single way to perform optimization. 
For small-input rewriting methods, its performance is good but may always get stuck into local optimal.
While the large-input rewriting methods' optimization ability can still be further optimized.
{\color{red}这一段值得好好写}

In this paper, we propose an efficient And-Inverter Graph (AIG) rewriting algorithm that utilizes four methods to expand the optimization search space on reconvergent cuts: pattern-rewriting, NPN-rewriting, exact synthesis, and SOP-rewriting.
The proposed algorithm selects the appropriate method to rewrite the MFFC at different scale by an evaluator to takes advantage of each method.
Additionally, we also propose a balance-aware cost estimation method to estimate the gain of the following delay optimization commands.
Our paper makes three contributions:
\begin{itemize}
    \item We propose an evaluator-based rewriting method which take advantage of the different rewrite methods;
    \item We propose a balance-aware cost estimation method to enhance the multiple optimization steps;
    \item We perform sufficient experiments for our proposed algorithm to show that our proposed algorithm expands the optimization search space with better quality. 
\end{itemize}

The rest of the paper is organized as follows.
Section~\ref{sec:preliminaries} summarizes the preliminaries of the rewriting method.
Section~\ref{sec:method} describes the detail about our evaluator-driven rewriting strategy.
The implementation are evaluated with sufficient experiment results in Section~\ref{sec:experiment}.
Finally, Section~\ref{sec:related_works} introduces some related works, and Section~\ref{sec:conclusion} concludes this paper.

==> sections/method.tex <==
\section{Method}
\label{sec:method}

In this section, we will provide a detailed description of our proposed method. 
Firstly, we will introduce the fundamental setup for the four rewriting methods. 
Secondly, we will present our evaluator-driven AIG rewriting strategy that integrates with a balance-aware cost estimation component. 
Lastly, we will explain the process of equivalent local replacement.

\subsection{Setup for the four rewrite methods}
\label{sec:method:main-rewrite-methods}
Our algorithm is based on the following four methods of rewriting, and we provide specifications for their use.
And the Fig. \ref{fig:4-rewrites} also shows the rough scheme for the four rewriting methods.
\begin{table}[htp]
\centering
\caption{The NPN classes for 2-6 inputs.}
\begin{tabular}{|c|cc|}
\hline
\#input & \#Boolean Functions & \#NPN classes  \\ \hline
2       & 16                  & 4              \\
3       & 256                 & 12             \\
4       & 65,536              & 222            \\
5       & 4,294,967,296       & 615,126        \\
6       & 1.84467E+19         & 2.00254E+14     \\ \hline
\end{tabular}
\end{table}

\begin{figure}[htp]
    \centering
    \includegraphics[scale=0.425]{figures/4-rewrites.pdf}
    \caption{{\color{red}不清晰,或者删除掉}
    Visualization of the four rewriting methods is presented, with a focus on the subgraph of the circuit and internal processing node: (a) denotes pattern rewriting scheme; (b) refers to cut enumeration-based rewriting algorithm; (c) represents exact synthesis scheme; and (d) indicates SOP minimization scheme.}
    \label{fig:4-rewrites}
\end{figure}

\subsubsection{Pattern-based rewrite}
Pattern-based rewrite method can be easily adopt to the less input Boolean structures. 
The patterns under three inputs are easier to exhaust, the patterns can be reduced further according to the symmetry of AND gate. Structure hash with checking to match the pattern.
% \begin{figure}[htp]
%     \centering
%     \includegraphics[scale=0.7]{figures/mffc-fencing.pdf}
%     \caption{Topological structures of the pattern rewriting under three-inputs. {\color{red}may not need here.}}
%     \label{fig:mffc-fencing}
% \end{figure}

\vspace{3pt}
\subsubsection{Cut enumeration-based rewrite} {\color{red}所有NPN-based换成cut enumeration}This approach is employed exclusively for input sizes not exceeding 4. It explores the NPN-equivalent space of the Boolean function through negating inputs, permuting inputs or negating output to seek the searched Boolean function's subgraph with best gain, while the depth constraints is also optional.
\subsubsection{Cache-based exact synthesis} The on-the-fly exact synthesis can be applied when the input size is no more than 5, and we use the cache-based exact synthesis for table-look up to reduce the runtime.
\subsubsection{SOP minimization} This method is mainly based on the iSOP minimization with large input sizes, and it is efficient to use SOP minimization when the input size is over 6. And we also limit the input size under 10 for a trade-off between time and optimization space.



\subsection{Proposed algorithm}

The proposed algorithm flow is shown in Fig. \ref{fig:flow}., it mainly consists of three steps: preprocessing, evaluator-driven minimization, replacement.
The rewrite algorithm is processed following the topological order. 
The dark node denoted the processed nodes as the root of MFFC, and it can also be the internal or leaves of the other node's MFFC; 
The white node denoted the unprocessed nodes; 
And the gray node denotes the current processing node as the root of a MFFC.

\vspace{5pt}
\begin{algorithm}
\small
\caption{Evaluator-driven AIG rewriting}
\label{algorithm:flow}
\begin{algorithmic}[1]
\Require Logic network $LG$
\Ensure Optimized logic network $LG'$
\State $V$ $\leftarrow$ topological\_sort($LG$)
\For{$n$ in $V$}
    \If{is\_logic\_gate($n$)}
        \State $cm$ $\leftarrow$ compute\_reconvergence\_driven\_mffc($n$)
        \State $tp$ $\leftarrow$ decide\_by\_evaluator($cm$)
        \State $ocm$ $\leftarrow$ optimize($tp$, $cm$)
        \State $mp$ $\leftarrow$ match\_ports($sg$, $cm$)
        \State local\_replace\_online($mp$, $ocm$)
    \EndIf
\EndFor
\State $LG'$ $\leftarrow$ remove\_dead\_nodes(LG)
\State \Return $LG'$
\end{algorithmic}
\end{algorithm}

And Algorithm \ref{algorithm:flow} provides a more detailed description.
First, we need to make a topological sort of the Logic network $LG$~(line 1). 
Because if we want to make a better gain, we would better process all the nodes following topological order.
Then, we will perform local rewrite for each node according the topological order $V$~(lines 2-10).
As for one logical node $n$ in $V$, the constrained MFFC is extracted from its constrained subgraph~(line 4).
Then, the evaluator will decide which rewrite method should be taken on according the feature of its ports and structures~(line 5).
% The corresponding Boolean function or Boolean algebra can also be computed by its leaves, internal nodes and root.
Then we will optimize the original MFFC structure $cm$ by the decided rewrite method through its Boolean function or Boolean algebra, and get the optimized subgrah $ocm$~(line 6).
And we will also acquire the ports matching information to make sure the replacement would be performed at the correct inputs or output~(line 7).
Finally, the new optimized subgraph $ocm$ need to replace the original $cm$ by the support of ports matching information $mp$, and one node has been processed done~(line 8).
After process all the nodes in $V$ following the steps above, the rewrite algorithm is terminal~(lines 11-12).

\subsection{MFFC computation}
MFFC is the key factor for rewriting algorithm.
As for the reconvergence-driven MFFC, reconvergent nodes will bring more opportunities for optimization.
So for we also compute the MFFC through the reconvergence-driven cut, and it results in reconvergence-driven MFFC.
\vspace{5pt}
\begin{algorithm}
\small
\caption{Constrained MFFC computation}
\label{algorithm:mffc}
\begin{algorithmic}[1]
\Require Logic network $LG$, 

node $n$
\Ensure Constrained MFFC $cm$
\State initialize two frontier lists $L_1$, $L_2$
\State $rc$ $\leftarrow$ compute\_reconvergent\_cut($n$)
\State $cm$.push(n)

\While {not\_visited\_all\_leaves($rc$)}
    \State remove\_duplicates($L_1$)
    \For{$nf$ in $L_1$}
        \If {is\_mffc\_node($nf$)}
            \For {$nc$ in FANINS($nf$)}
                \State $L_2$.push($nc$)
            \EndFor
            $cm$.push($nc$)
        \EndIf
    \EndFor
    \State $L_1$ $\leftarrow$ $L_2$
    \State $L_2$.clear()
\EndWhile
\State \Return $cm$
\end{algorithmic}
\end{algorithm}

Algorithm \ref{algorithm:mffc} shows the algorithm of constrained MFFC computation.
This algorithm is based on bread first search~(BFS) to collect the nodes from root to leaves.
Firstly, we initialize two lists $L_1$ and $L_2$, $L_1$ is the working list and $L_2$ is a temporary list to collect fanins~(line 1).
Secondly, the reconvergent cut $rc$ is computed for the multi-inputs and signal output subgraph to constraint the space of MFFC~(line 2).
Then, we will collect the constrained MFFC $cm$ by BFS from root to leaves of $rc$. If the fanouts of node $nf$ is all included in $cm$, we make it a mffc node of $cm$, and is\_mffc\_node($nf$) return true.
We add the fanins of $nf$ to $L_2$ for the next iteration until all the leaves of $rc$ are visited~(lines 4-15).
Lastly, $cm$ is complete and returned.


\subsection{Evaluator-driven minimization}
The four main rewriting algorithms and their setup are discussed in Section \ref{sec:method:main-rewrite-methods} above. 
Additionally, Table \ref{tab:range} provides a visual representation of the input range for these algorithms.

\subsubsection{Decision}
\begin{table}[htp]
\centering
\caption{Decision with input range}
\label{tab:range}
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{algorithms}} & \multicolumn{1}{c|}{\textbf{input range}} \\ \hline
                     pattern-rewriting    &      [2,4)                                \\
                     NPN-rewriting        &      4                                    \\
                     exact-synthesis      &      5                                    \\
                     SOP minimization     &      (5,10]                               \\ \hline
\end{tabular}
\end{table}
As shown in Table \ref{tab:range}, we have tailored the input range for each rewriting algorithm to ensure runtime and quality tradeoff.
The pattern-rewriting technique is appropriate for input sizes up to 3; the NPN-based rewriting method is suitable for input sizes of 4; exact synthesis is applicable for input sizes below 5, while SOP minimization is recommended for input sizes exceeding 6.
Therefore, the rewriting algorithm can be effectively applied for input sizes up to 10.

\subsubsection{Minimization}
The minimization process is executed through their proprietary optimization algorithm. We will outline the approach for maintaining depth and area in accordance with the target optimization strategy.
\begin{itemize}
    \item \textbf{Preserve depth by nonnegative slack}\cite{daomap}. 
    The slack of node $n$ is defined as: $$slack(n)=require(n)-arrive(n).$$
    And Code 1 shows the arrival time and require time computation by unit delay model.
    The arrival time can be computed as the max depth from PIs to $n$, and the required time can be computed by the max depth of POs minus the depth between $n$ and the max depth's PO node. 
    So if the slack for the newly optimized subgraph is nonnegative, the circuit's depth will be preserved.
    \item \textbf{Preserve area by fast area estimation}. 
    Because of the fanout size refers to the number that it is used, so we can record the changged fanout size of current subgraph to evaluate the area gain, and the gain can be computed by: $$area\_gain= deref\_cut(n, cut) - ref\_cut(n, cut') .$$
    The ref\_cut and deref\_cut algorithm as shown in Code 2 can perform fast area cost estimation for the newly optimized subgraph.
    The ref refers to reference, it means that inserting a subgraph into graph, and the deref refers to dereference, it means that remove a subgraph from graph.
    Each node will be initialized the $ref$ by node's fanout size.

\end{itemize}

\
\
\


% \begin{lstlisting}[caption=arrive time and require time computation by unit delay model]
% Void compute_arrive_time(aig) {
%     for n in aig do
%         arrive(n) = 0;
%     order = topological_order(aig)
%     for n in order do
%         for nc in children(n) do
%             arrive(n) = max(arrive(n), arrive(nc)+1)
% }
% Void compute_required_time(aig) {
%     arrive_max = get_max_arrive_time(POs);
%     for n in aig do
%         require(n) = +;
%     for po in POs do
%         require(n) = arrive_max;
%     rorder = reverse_topological_order(aig)
%     for n in rorder do
%         for nc in children(n) do
%             require(nc) = min(require(nc), require(n)-1)
% }
% \end{lstlisting}


% \begin{lstlisting}[caption=reference and dereference algorithms]
% Integer	ref_cut(n, cut) {
%     if (n in cut)
%         return 0;
%     value = 1;
%     fanins = FANINs(n);
%     for nf in  fanins do
%         ref(nf) = ref(nf) + 1;
%         if(ref(nf) == 1)
%             value += ref_cut(nf, cut);
%     return value;
% }             	            	 
% Integer	deref_cut(n, cut) {
%     if (n in cut)
%         return 0;
%     value = 1;
%     fanins = FANINs(n);
%     for nf in  fanins do
%         ref(nf) = ref(nf) - 1;
%         if(ref(nf) == 0)
%             value += deref_cut(nf, cut);
%     return value;
% }             
% \end{lstlisting}


\begin{figure}[htp]
    \centering
    \includegraphics[scale=0.35]{figures/balance.pdf}
    \caption{AIG balancing through AND-cover.}
    \label{fig:balance}
\end{figure}

\subsubsection{Balance-aware cost estimation}
% The optimization ability of a single optimization algorithm is often limited. In logic synthesis, multiple optimization operators facing different objectives are usually used together to achieve a desired optimization result.
% The rewriting algorithm is often used multiple times in succession with the balance operator to perform a mix of area and depth optimizations.
% Hence, we proposed a heuristic balance-aware cost estimation method to make the result of rewriting following by balance will have a lesser depth, and the balance-aware cost function of a subgraph is as the following:
% $$ 
%     cost = \frac{\#NE}{\#PE+\#NE} \cdot \sum_{i=1}^{c} \frac{CoverLevel_i \cdot CoverDepth_i}{CoverSize_i}
% $$

% This cost function is based on the scheme of and-balancing algorithm\cite{sop-balance-iccad11} in AIG.
% The \# symbol means ``the number of", $NE$ means the inverter edge, $PE$ means the non-inverter edge.
% The and-balancing algorithm benefits from the theory that multi-inputs AND gates can be generated by the two-input AND tree. 
% And as shown in Fig. \ref{fig:balance}., an \textit{AND-cover} is an AND-tree that there is no inverter edge between any two AND gates.


% \vspace{5pt}
% \begin{algorithm}
% \small
% \caption{Fast cost estimation of tree-balance}
% \label{algorithm:balance}
% \begin{algorithmic}[1]
% \Require Single output Cone $cut$
% \Ensure Estimated cost $value$

% \end{algorithmic}
% \end{algorithm}


\subsection{Local replacement}
As there are two paradigms for rewrite: Boolean-equivalence-based and Boolean-matching-based, the local replacement algorithm need to be brought up after the minimization.
The local replacement is based on the matching information of ports, i.e. the leaves and root of MFFC.
And the matching information is consisted of permutation and phase.
The permutation mainly provides the transformed order of inputs, and the phase mainly provides the negation information of inputs and outputs.

\vspace{5pt}
\begin{algorithm}[htp]
\small
\caption{Online local replacement}
\label{algorithm:replacement}
\begin{algorithmic}[1]
\Require Logic Network $LG$,

Constrained MFFC $cm$,

Optimized subgraph $ocm$,

Matching $mp$
\Ensure Gain $v$
\State $phase$ $\leftarrow$ extract\_phase($mp$)
\State $perm$ $\leftarrow$ extract\_permutation($mp$)
\State matching\_inputs\_by\_permutation($cm$, $ocm$, $perm$)
\State matching\_inputs\_by\_phase($cm$, $ocm$, $phase$)
\State matching\_output\_by\_phase($cm$, $ocm$, $phase$)
\State $v_1$ $\leftarrow$ deref\_subgraph($cm$)
\State insert\_optimized\_subgraph($LG$, $ocm$)
\State $v_2$ $\leftarrow$ ref\_subgraph($ocm$)
\State deref\_subgraph($ocm$)
\State ref\_subgraph($cm$)
\State $LG'$ $\leftarrow$ remove\_original\_mffc($LG$, $cm$)
\State \Return $v_1$ - $v_2$
\end{algorithmic}
\end{algorithm}

Algorithm \ref{algorithm:replacement} shows the flow of the online local replacement algorithm.
The first step is to extract the permutaiton $perm$ and phase $phase$ to match the inputs and output before and after optimization~(lines 1-5).
Then, the optimized subgraph should be generated from leaves to root in the original logic network $LG$ according to $perm$ and $phase$~(line 6).
Only in this way, we are able to guarantee that the connection relation between the logic gates is correct, and the correct inverter gate is also added to ensure the correctness of the logic.
Following the aforementioned steps, it is necessary to eliminate the initial internal nodes in MFFC by removing their fanout signals to become a dead node~(line 7), and the online local replacement algorithm is terminal.

\begin{figure}
    \centering
    \includegraphics[scale=0.8]{figures/example.pdf}
    \caption{Example of AIG rewriting.}
    \label{fig:example}
\end{figure}

\begin{example}
The Fig. \ref{fig:example} shows the example of AIG rewriting. 
Firstly, the original subgraph will be evaluated by our evaluator to decide which rewriting algorithm is better, then we will get the optimization result.
Secondly, we will make a fast area cost estimation by ``ref\_cut'' and ``deref\_cut'' algorithm.
The ``deref\_cut'' algorithm will estimate the area cost value for the origianl cut is 2, and the ``ref\_cut'' algorithm will estimate the area cost value for the candidate is 1.
Therefore the area gain for the newly optimization subgraph is 1.
For logic equivalence, we will correctly insert the newly sugraph by teh port matching.
\end{example}



==> sections/preliminary.tex <==
\section{preliminaries}
\label{sec:preliminaries}

In this section, we provide a summary of the related definitions for rewrite, with a focus on Boolean function, Boolean algebra and Boolean network. There is also an example to illustrates our motivation.
Additionally, we introduce two paradigms of equivalence: Boolean equivalence and Boolean matching.

\subsection{Notations and basic definitions}
\subsubsection{Boolean algebra/function}
A $Boolean\ variable$ is a variable that take on values only from the set $B$=$\{0,1\}$.
The $Boolean\ algebra$ deals with Boolean variables and logic operations.
An $n$-input and single-output $Boolean\ function$ $f(X):B^{n}\to B$, $B$=$\{0,1\}$, where $X$=$(x_{1},x_{2},...,x_{n})$,$x_{i}\in B$,$1\leq i \leq n$ is a vector of input Boolean variables with size $n$. And the truth table of $f(X)$ is defined as $T(f)=(f(X_{2^n-1}),...,f(X_{(1)}),f(X_{(0)}))$ is a binary vector with size $2^n$.
\subsubsection{Boolean network}
A $Boolean\ network$ is modeled as a directed acycilc graph~(DAG), where the node denotes a logic gate, input or output and an edge denotes a signal wire between two logic gates.
Let $G(V,E)$ be a Boolean network with the node set $V=\{v_1, v_2, ..., v_n\}$ which is composed of input set, output set and function set. And the input set defines as $I=\{v_i\ is\ the\ input|v_i\in V\}$, the output set defines as $O=\{v_i\ is\ the\ output|v_i\in V\}$, and the function set defines as $F=\{v_i\ is\ the\ internal\ logic\ gate|v_i\in V\}$. Thus, we can get $V=I\cup O\cup F$. And the edge set can be defined as $E\{(v_i,v_j)|v_i,v_j\in V\}$. 

A node $v$ has zero or more $fanins$ and $fanouts$, and fanins mean the nodes that flowed in and fanouts mean the nodes that flowed out. 
The $primary\ inputs$~(PIs) are the nodes that have zero fanins, and the $primary\ outputs$~(POs) are the nodes that have zero fanouts, we can intuitively think of PIs and POs are the inputs and outs of the circuit. 
The node $v$ is $dead$ \textit{iff} it is an internal logic gate without any fanouts.
A $transitive\ fanin/fanout\ cone$~(TFI/TFO) of the node $v$ is a subset of nodes that reachable through the fanin/fanout edges of $v$. 
If there is a path from node $v_i$ to $v_j$, then we can say $v_i$ is in the TFI of $v_j$, and $v_j$ is in the TFO of $v_i$.
A $max\ fanout\ free\ cone$~(MFFC) of the node $v$ is a subset of the TFI of $v$, such that each path from a node in this subset to the POs must passes through $v$. A node is the $leaf$ of MFFC which its TFI does not include any nodes in MFFC, and $v$ is the $root$ of MFFC. 
A cut $c$ of node $v$ is a set of nodes whose TFI must flow to $v$, in short, $c$ are the leaves, and $v$ is the root for $c$.
The $k$-feasible cut is the cut that leaves' size within $k$.
And And-Inverter Graph~(AIG) is a Boolean network with the internal nodes refer to AND gate and the edges refer to inverter-embed signal or not.

\subsubsection{Reconvergence-driven cut}

{\color{red} need more details.}
The $reconvergence$ refers to that the paths starting at the fanout of a node $n$ will meet again before arriving the POs. 
And it is inevitable due to the logic sharing in multi-level Boolean networks.
The $reconvergence{-}driven\ cut$ technique works by identifying points in the circuit where multiple paths converge and then diverge again. 
These points are known as $reconvergence\ points$, and they often represent opportunities for optimization.

\subsection{Motivation example}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth, height=0.185\textheight]{figures/motivation-example.pdf}
    \caption{Motivation example for rewriting at different scales.{\color{red}给一个例子，三种优化方式不同，优化力度不同}}
    \label{fig:motivation}
\end{figure}

\begin{figure*}[htbp]
    \centering
    \includegraphics[scale=0.48]{figures/method-flow.pdf}
    \caption{Our method flow for cone-evaluation-driven rewriting strategy.}
    \label{fig:flow}
\end{figure*}

\begin{table}
\centering
\caption{Statistic the distribution of cut size in real circuits}
\begin{tabular}{|l|l|llll|}
\hline
\multicolumn{1}{|l|}{case} & \multicolumn{1}{l|}{size} & \multicolumn{1}{l|}{\#3-input} & \multicolumn{1}{l|}{\#4-input} & \multicolumn{1}{l|}{\#5-input} & \multicolumn{1}{l|}{\#6-input} \\ \hline
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\
                        &                           &                                &                            &                              &                            \\ \hline
\end{tabular}
\end{table}

\begin{figure}
\centering
\subfigure[$f = \overline{x_1} + x_2\overline{x_3}$]{
    \label{fig:a}
    \includegraphics[width=0.4\linewidth]{figures/two-paradiam-a.pdf}
    } \\
\subfigure[$g = x_1x_2 + x_3$]{
    \label{fig:b}
    \includegraphics[width=0.4\linewidth]{figures/two-paradiam-b.pdf}
    }
\subfigure[$h = x_1(\overline{x_2}+x_3)$]{
    \label{fig:c}
    \includegraphics[width=0.4\linewidth]{figures/two-paradiam-c.pdf}
    }
\caption{The two paradigms of equivalence: (a) and (b) are NPN-equivalent; (a) and (c) are Boolean-equivalent.}
\label{fig:two-paradigms}
\end{figure}

The Fig. \ref{fig:motivation} illustrates the circuit rewriting at different scales on the reconvergent cut. 
It should be noted that due to distinct optimization methods, the strength of optimization varies across different scales.
Therefore, our motivation is to select the appropriate rewriting algorithm for optimization according to the scale and structural characteristics of the reconvergent cut, so as to improve the optimization ability.

\subsection{Two paradigms of equivalence}
There are two paradigms of equivalence for local replacement: the Boolean-equivalence-based equivalence that preserves inputs and output, while the Boolean-matching-based equivalence that may alter the input order or introduce inverter gates at inputs or output.

\subsubsection{Boolean equivalence-based equivalence}
Boolean algebra minimization is the representative of Boolean equivalence\cite{logical-equivalence}.
We can say that two Boolean algebra $f$ and $g$ are Boolean equivalent \textit{iff} their Boolean function are equivalent.
In the process or Boolean algebra minimization, the literals and clauses of the expression can be removed to reduce the cost while remain the inputs and output unmodified. 
So it is easy to replace the original MFFC directly by the newly optimized MFFC.

\subsubsection{Boolean matching-based equivalence}
Boolean matching\cite{Boolean-matching} is a verification problem of that whether we can find a matching relation for two sub-circuits inputs and outputs. 
We focus on the multi-input and signal-output sub-circuits here, and NPN classification is the representation here.
We can say two single-output Boolean functions $f$ and $g$ are NPN-equivalent if we find a transformation function $\Delta$ on inputs and output for $f$ to get that $\Delta(f) = g$.
Therefore, we can perform the equivalent local replacement iff we find the transformation function $\Delta$ between $f$ and $g$.

\begin{example}    
As shown in Fig.\ref{fig:two-paradigms}., $f$ and $g$ are NPN equivalent because of $f(\overline{x_3}, x_2, \overline{x_1})=g(x_1,x_2,x_3)$, the transformation procedures are swapping $x_1$ and $x_3$, then negating them.
And $f$ and $h$ are Boolean equivalent with the same Boolean function $(10100010)_2$.
\end{example}

\subsection{Q-learning}


==> sections/related_works.tex <==
\section{related works}
\label{sec:related_works}
\subsubsection{pattern rewriting}
\begin{itemize}
    \item \textbf{pros}: Thanks to its rule-based rewriting scheme, patter rewriting algorithm can obtain relatively fast replacement with fewer inputs and simple structures. 
    \item \textbf{cons}: However, its local optimization ability remains insufficient for practical applications.
\end{itemize}

\subsubsection{NPN rewriting}
\begin{itemize}
    \item \textbf{pros}: The optimization quality is enhanced by the large search space achieved through cut enumeration of the fanin cones from different fanins combination.
    \item \textbf{cons}: The extensive exploration of its optimization space also make it difficult to extend beyond 4-input cuts.
\end{itemize}

\subsubsection{exact synthesis}
\begin{itemize}
    \item \textbf{pros}: It can provide the optimal area or delay cost by encoding Boolean function to Boolean chain and checking equivalence by SAT solver.
    \item \textbf{cons}: Moreover, the encoding and checking processes consume a significant amount of time, rendering it inefficient for processing large input subgraphs.
\end{itemize}

\subsubsection{SOP minimization}
\begin{itemize}
    \item \textbf{pros}: The algorithm is proficient in optimizing subgraph with large inputs.
    \item \textbf{cons}: The optimization result cannot be compared with the other three.
\end{itemize}

